Spectrum-Flexible Secure Broadcast Ranging

Secure ranging is poised to play a critical role in several emerging applications such as self-driving cars, unmanned aerial systems, wireless IoT devices, and augmented reality. In this paper, we propose a design of a secure broadcast ranging systems with unique features and techniques. Its spectral-flexibility, and low-power short ranging bursts enable co-existence with existing systems such as in the 2.4GHz ISM band. We exploit a set of RF techniques such as upsampling and successive interference cancellation to achieve high accuracy and scalability to tens of reflectors even when operating over narrow bands of spectrum. We demonstrate that it can be implemented on popular SDR platforms FPGA and/or hosts (with minimal FPGA modifications). The protocol design, and cryptographically generated/detected signals, and randomized timing of transmissions, provide stealth and security against denial of service, sniffing, and distance manipulation attacks. Through extensive experimental evaluations (and simulations for scalability to over 100 reflectors) we demonstrate an accuracy below 20cm on a wide range of SNR (as low as 0dB), spectrum 25MHz-100MHz, with bursts as short as 5us.

==> macros-protocol.tex <==

% \usepackage{import}
% \import{.}{pgfmoduleplot.code.tex}
% \usepackage[
%     n, % or  lambda
%     advantage,
%     operators,
%     sets,
%     adversary,
%     landau,
%     probability,
%     notions,
%     logic,
%     ff,
%     mm,
%     primitives,
%     events,
%     complexity,
%     oracles,
%     asymptotics,
%     keys
%     ]{ cryptocode }

\usepackage{cryptocode}

